An inclusive search for the Higgs boson in the four-lepton final state at CDF

An inclusive search for the standard model Higgs boson using the four-lepton final state in proton-antiproton collisions produced by the Tevatron at sqrt(s) = 1.96 TeV is conducted. The data are recorded by the CDF II detector and correspond to an integrated luminosity of 9.7 /fb. Three distinct Higgs decay modes, namely ZZ, WW, and tau-tau, are simultaneously probed. Nine potential signal events are selected and found to be consistent with the background expectation. We set a 95% credibility limit on the production cross section times the branching ratio and subsequent decay to the four lepton final state for hypothetical Higgs boson masses between 120 GeV/c^2 and 300 GeV/c^2.

==> biblio.tex <==
\begin{thebibliography}{99}

\bibitem{MSSM}
M.~Carena, S.~Heinemeyer, C.~E.~M.~Wagner and G.~Weiglein, arXiv:hep-ph/0202167.

\bibitem{techni}
C.~T.~Hill and E.~H.~Simmons, arXiv:hep-ph/0203079.

\bibitem{mjjme}  T.~Aaltonen {\it et al.} (CDF Collaboration), Phys. Rev. Lett. {\bf 104}, 101801 (2010); http://www-cdf.fnal.gov/physics/ewk/2010/WW\_WZ/index.html.

%J/psi and B hadron production PRD -- detector description
\bibitem{CDFdet} D. Acosta {\it et al.} (CDF Collaboration), Phys. Rev. D {\bf 71}, 032001 (2005).

\bibitem{coord} We use a cylindrical coordinate system with its origin in the center 
of the detector, where $\theta$ and $\phi$ are the polar and azimuthal angles, respectively,
and pseudo-rapidity is $\eta= - \rm ln$ $\rm tan(\theta/2)$. 
The transverse energy $E_T$ (momentum $p_T$) is defined as $E\sin\theta$ ($p\sin\theta$).
The missing $E_T$ ($\METVEC$) is defined by $\METVEC = -\sum_iE_T^i{\hat n}_i$,
where ${\hat n}_i$ is a unit vector perpendicular to the beam axis and pointing at the $i^{th}$ calorimeter tower.  
~$\METVEC$ is corrected for high-energy muons and also jet energy corrections.
We define $\MET=|\METVEC|$. The transverse mass of the $W$ is defined as $M_T (W)=\sqrt{2p_T^l \MET (1-\cos(\Delta \phi^{l\nu}))}$.

\bibitem{lumi} D.~Acosta {\it et al.}, Nucl.\ Instrum.\ Methods A {\bf494}, 57 (2002).

\bibitem{isolation} Lepton isolation ($Iso$) is defined as $\frac{\sum E_T}{E_T}$, $\frac{\sum E_T}{p_T}$ for electrons and muons respectively, where $\sum E_T$ is the calorimetric energy in a cone 0.4 around the lepton.

\bibitem{jet_details} A. Bhatti {\it et al.}, Nucl.\ Instrum.\ Methods A {\bf 566}, 375 (2006).

\bibitem{cdfsim} E.~Gerchtein, M.~Paulini (2003), arXiv:physics/0306031.
\bibitem{pythia} T.~Sj\"ostrand {\it et al.}, Comput.\ Phys.\ Commun., {\bf 135},\
 238 (2001).

\bibitem{alpgen} M.~L.~Mangano {\it et al.}, J.\ High\ Energy\ Phys.\ 07 (2003) 001.

\bibitem{MLM} S. Hoche {\it et al.}, arXiv:hep-ph/0602031v1.

\bibitem{tesi} V.~Cavaliere, Ph.D. Thesis.  University of Siena, FERMILAB-THESIS-2010-51 (2010).

\bibitem{mesxs} T.~Aaltonen {\it et al.}, (CDF Collaboration),  Phys. Rev. Lett. {\bf 100}, 102001 (2008).
%\prl{100}{2008}{102001}
%
%D.~Acosta {\it et al.} (CDF collaboration), Phys. Rev. Lett. {\bf 94}, 091803 (2005).

\bibitem{theoxs} M.~Cacciari {\it et al.}, J.\ High\ Energy\ Phys.\ 09 (2008) 127; B.~W.~Harris {\it et al.}, Phys.\ Rev.\  D {\bf 66}, 054024 (2002); J.M. Campbell and R.K. Ellis, Phys.\ Rev.\ D {\bf 60}, 113006 (1999).  

\bibitem{KStest} The reported KS probability corresponds to the KS test between data and background distributions. It does not account for the fact that the background distributions are constrained by fits to data. The reported values are thus an upper limit on KS probability.

\bibitem{mcfm1} J.~M.~Campbell and R.~K.~ Ellis, Phys.\ Rev.\ D{\bf 62}, 114012 (2000).

\bibitem{mcfm2} MCFM, http://mcfm.fnal.gov.

\bibitem{Higgs_xsec_and_BR} T.~Han and S.~Willenbrock, Phys.\ Lett.\ B{\bf 273} (1991) 167;
A.~Djouadi, J.~Kalinowski and M.~Spira, Comp.\ Phys.\ Commun. {\bf 108} C (1998) 56, hep-ph/9704448.

\bibitem{Higgs} T.~Aaltonen {\it et al.}, (CDF Collaboration),  Phys. Rev. Lett. {\bf 103}, 101802 (2009).

\bibitem{M_lnujj} $M_{({\rm lepton},\nu,jj)}$ denotes the total invariant mass of the lepton, neutrino and dijet system. We reconstruct the longitudinal component of the neutrino momentum by imposing a $W$ mass of 80.398~GeV/$c^2$. We consider both real solutions for the $p_z$ of the neutrino  and we discard complex solutions of the $W$ mass equation.








%\bibitem{web} Web Page

%%    \bibitem{hagiwara} K. Hagiwara, S. Ishihara, R. Szalapski, and D. Zeppenfeld, Phys. Rev. D {\bf 48}, 2182 (1993).
%%    
%%    \bibitem{diblepCDF} D. Acosta {\it et al.} (CDF Collaboration), Phys. Rev. Lett. {\bf 94}, 211801 (2005); 
%%    A. Abulencia {\it et al.} (CDF Collaboration), {\it ibid} {\bf 98}, 161801 (2007); 
%%    T. Aaltonen {\it et al.} (CDF Collaboration), {\it ibid} {\bf 100}, 201801 (2008).
%%    
%%    \bibitem{diblepD0} V.M. Abazov {\it et al.} (D0 Collaboration), Phys. Rev. Lett. {\bf 94}, 151801 (2005) and Phys. Rev. D {\bf 76}, 111104(R) (2007).
%%    
%%    \bibitem{d0lvjj} V. M. Abazov {\it et al}. (DO \ collaboration), Phys. Rev. Lett. {\bf 102}, 161801 (2009).
%%    
%%    \bibitem{cdflvjj} T.~Aaltonen {\it et al.} (CDF Collaboration), Phys. Rev. D {\bf 79}, 112011 (2009).
%%    
%%    \bibitem{cdfmetjj}  T.~Aaltonen {\it et al.}  (CDF Collaboration),
%%     %``First Observation of Vector Boson Pairs in a Hadronic Final State at the
%%     %Tevatron Collider,''
%%     Phys.\ Rev.\ Lett.\  {\bf 103}, 091803 (2009).
%%    % [arXiv:0905.4714 [hep-ex]].
%%    
%%    
%%    \bibitem{WHME}  T.~Aaltonen {\it et al.}  (CDF Collaboration),
%%     %``Search for a Higgs Boson in $W H \to \ell \nu b \bar{b}$ in $p\bar{p}$
%%     %Collisions at $\sqrt{s} = 1.96$ TeV,''
%%     Phys.\ Rev.\ Lett.\  {\bf 103}, 101802 (2009).
%%    % [arXiv:0906.5613 [hep-ex]].
%%    
%%    
%%    \bibitem{cdfsingletop}  T.~Aaltonen {\it et al.}  (CDF Collaboration),
%%     %``Measurement of the Single Top Quark Production Cross Section at CDF,''
%%     Phys.\ Rev.\ Lett.\  {\bf 101}, 252001 (2008);
%%    %[arXiv:0809.2581 [hep-ex]].
%%     T.~Aaltonen {\it et al.}  (CDF Collaboration),
%%     %``Observation of Electroweak Single Top Quark Production,''
%%     Phys.\ Rev.\ Lett.\  {\bf 103}, 092002 (2009).
%%    
%%    \bibitem{pdong} P. Dong, Ph.D. thesis, University of California, Los Angeles, FERMILAB-THESIS-2008-12 (2008).
%%    
%%    \bibitem{madevent} J.~Alwall {\it et al.}, J.\ High\ Energy\ Phys.\ 09 (2007) 028.
%%    
%%    
%%    \bibitem{CTEQ} J. Pumplin {\it et al.}, J.\ High\ Energy\ Phys.\ 07 (2002) 012.
%%    
%%    \bibitem{madgraph} F.~Maltoni and T.~Stelzer, J.\ High\ Energy\ Phys.\ 02 (2003) 027.
%%    
%%    \bibitem{lyons1988} L.~Lyons, D.~Gibaut, and P.~Clifford, Nucl.\ Instrum.\ Methods A {\bf 270}, 110 (1988).
%%    
%%    \bibitem{VVtheory} J.~M.~Campbell and R.~K.~Ellis, Phys.\ Rev.\ D {\bf 60}, 113006 (1999).
%%    
%%    %\bibitem{trigger} T. Aaltonen {\it et al.} (CDF Collaboration), Phys.\ Rev.\ Lett.\  {\bf 100}, 211801 (2008).
%%    
%%    %\bibitem{secvtx} D. Acosta {\it et al.}, Phys. Rev. D {\bf 71}, 052003 (2005).
%%    
%%    %\bibitem{jesnim} A. Bhatti {\it et al.}, Nucl. Instrum. Methods A {\bf 566}, 2 (2006).
%%    
%%    %\bibitem{pythia} T.~Sj\"ostrand {\it et al.}, Comput. Phys. Commun, {\bf 135}, 238 (2001).
%%    
%%    % for version 6.4 -- we do not use this but it's a more recent document.
%%    %\bibitem{pythia} T.~Sj\ostrand, S.~Mrenna and P.~Skands, JHEP {\bf 05}, 026 (2006).
%%    
%%    %\bibitem{ttbarxs} R. Bonciani {\it et al.}, Nucl.\ Phys.\ B {\bf 529}, 424 (1998); 
%%    %M. Cacciari {\it et al.}, J.\ High\ Energy\ Phys. {\bf 0404}, 068 (2004). 
%%                                        
%%      
%%    %\bibitem{alpgen} M.~L.~Mangano {\it et al.}, J.\ High\ Energy\ Phys {\bf 0307}, 001 (2003);
%%    %M.~L.~Mangano {\it et al.}, Nucl. Phys. B {\bf 632} 343 (2002);
%%    %F.~Caravaglios {\it et al.}, Nucl. Phys. B {\bf 539}, 215 (1999).
%%    
%%    %\bibitem{CTEQ} J. Pumplin {\it et al.}, J.\ High\ Energy\ Phys. {\bf 0207}, 012 (2002).
%%    
%%    %\cite{Hocker:2007ht}
%%    %\bibitem{TMVA}
%%    %  A.~H\"ocker {\it et al.},
%%    %  %``TMVA: Toolkit for multivariate data analysis,''
%%    %  PoS A {\bf CAT}, 040 (2007)
%%    %  [arXiv:physics/0703039].
%%    
%%    %\cite{Amsler:2008zz}
%%    %\bibitem{pdg}
%%    %  C.~Amsler {\it et al.}  [Particle Data Group],
%%    %  %``Review of particle physics,''
%%    %  Phys.\ Lett.\  B {\bf 667}, 1 (2008).
%%    %  %%CITATION = PHLTA,B667,1;%
%%    
%%    
\end{thebibliography}


==> figures_tables/Limit_H4l_97.tex <==
%\begin{tabular}{|l|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|}
\begin{tabular}{lrrrrrrrrrrrrrrrrrrr}
%\hline
H$\to$4$\ell$   &         120 &         130 &         140 &         150 &         160 &         170 &         180 &         190 &         200 &         210 &         220 &         230 &         240 &         250 &         260 &         270 &         280 &         290 &         300 \\
\hline
%     $-2\sigma/\sigma_{SM}$ &       29.1 &       15.1 &        9.2 &        7.9 &       12.2 &       17.9 &       13.1 &        5.9 &        6.0 &        7.9 &        9.6 &       10.3 &       11.6 &       12.7 &       14.0 &       15.2 &       16.0 &       18.3 &       20.0 \\
%     $-1\sigma/\sigma_{SM}$ &       31.2 &       16.2 &        9.7 &        8.1 &       12.8 &       19.6 &       14.0 &        7.3 &        7.9 &        9.7 &       11.3 &       12.5 &       12.9 &       14.7 &       16.0 &       18.0 &       18.0 &       20.6 &       22.4 \\
   $\mathrm{Expected}/\sigma_{SM}$ &    38.0 &    18.3 &    11.7 &     9.4 &    16.0 &    25.1 &    18.5 &     9.8 &    10.6 &    12.9 &    15.7 &    16.6 &    18.9 &    20.5 &    21.1 &    23.2 &    23.5 &    28.0 &    30.5 \\
%   $\mathrm{Median}/\sigma_{SM}$ &    38.0 &    18.3 &    11.7 &     9.4 &    16.0 &    25.1 &    18.5 &     9.8 &    10.6 &    12.9 &    15.7 &    16.6 &    18.9 &    20.5 &    21.1 &    23.2 &    23.5 &    28.0 &    30.5 \\
%   $ \bf Median/\sigma_{SM}$ & \bf   38.0 & \bf   18.3 & \bf   11.7 & \bf    9.4 & \bf   16.0 & \bf   25.1 & \bf   18.5 & \bf    9.8 & \bf   10.6 & \bf   12.9 & \bf   15.7 & \bf   16.6 & \bf   18.9 & \bf   20.5 & \bf   21.1 & \bf   23.2 & \bf   23.5 & \bf   28.0 & \bf   30.5 \\
\hline
% $\bf Observed/\sigma_{SM}$ & \bf   42.4 & \bf   20.5 & \bf   12.6 & \bf    9.5 & \bf   16.8 & \bf   28.5 & \bf   16.3 & \bf    8.2 & \bf    7.2 & \bf    7.9 & \bf   10.3 & \bf   20.5 & \bf   21.1 & \bf   17.4 & \bf   17.3 & \bf   18.2 & \bf   19.9 & \bf   24.1 & \bf   28.6 \\
 $ \mathrm{Observed}/\sigma_{SM}$ &    42.4 &    20.5 &    12.6 &     9.5 &    16.8 &    28.5 &    16.3 &     8.2 &     7.2 &     7.9 &    10.3 &    20.5 &    21.1 &    17.4 &    17.3 &    18.2 &    19.9 &    24.1 &    28.6 \\
%\hline
\end{tabular}


==> pacs.tex <==
\pacs{14.80.Bn, 11.15.Ex}

